Formal Safety and Security Assessment of an Avionic Architecture with Alloy

We propose an approach based on Alloy to formally model and assess a system architecture with respect to safety and security requirements. We illustrate this approach by considering as a case study an avionic system developed by Thales, which provides guidance to aircraft. We show how to define in Alloy a metamodel of avionic architectures with a focus on failure propagations. We then express the specific architecture of the case study in Alloy. Finally, we express and check properties that refer to the robustness of the architecture to failures and attacks.

==> eptcsdata.tex <==
\providecommand{\firstpage}{8}
\providecommand{\publicationstatus}{J. Pang and Y. Liu (Eds.): 3rd International Workshop\\ on Engineering Safety and Security Systems 2014 (ESSS 2014)\\
EPTCS 150, 2014, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.150.2}{10.4204/EPTCS.150.2}}
\pdfoutput=1

